Learning Graph Embedding with Adversarial Training Methods

Graph embedding aims to transfer a graph into vectors to facilitate subsequent graph analytics tasks like link prediction and graph clustering. Most approaches on graph embedding focus on preserving the graph structure or minimizing the reconstruction errors for graph data. They have mostly overlooked the embedding distribution of the latent codes, which unfortunately may lead to inferior representation in many cases. In this paper, we present a novel adversarially regularized framework for graph embedding. By employing the graph convolutional network as an encoder, our framework embeds the topological information and node content into a vector representation, from which a graph decoder is further built to reconstruct the input graph. The adversarial training principle is applied to enforce our latent codes to match a prior Gaussian or Uniform distribution. Based on this framework, we derive two variants of adversarial models, the adversarially regularized graph autoencoder (ARGA) and its variational version, adversarially regularized variational graph autoencoder (ARVGA), to learn the graph embedding effectively. We also exploit other potential variations of ARGA and ARVGA to get a deeper understanding on our designs. Experimental results compared among twelve algorithms for link prediction and twenty algorithms for graph clustering validate our solutions.

==> bio.tex <==
\vspace{-1cm}
	\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{small_pics/shirui.png}}]{Shirui Pan}
		Shirui Pan received the Ph.D. degree in computer science from the University of Technology Sydney (UTS), Ultimo, NSW, Australia. He is a Lecturer with the Faculty of Information Technology, Monash University, Australia.  His
		research interests include data mining and machine
		learning. To date, Dr Pan has published over 60 research papers in top-tier journals and conferences, including the IEEE Transactions on Neural Networks and Learning Systems (TNNLS), IEEE Transactions on Knowledge and Data Engineering (TKDE), and IEEE Transactions on Cybernetics (TCYB).
	\end{IEEEbiography}
	
	\vspace{-1cm}
	\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{small_pics/Ruiqi_HU.JPG}}]{Ruiqi Hu}
		received the Ph.D. degree in computer science from the University of Technology Sydney (UTS), Ultimo, NSW, Australia. He is currently a Research Associate in the Centre for Artificial Intelligence (CAI), UTS. His research concentrates on data mining and graph embedding. His recent works have been accepted by top-tier conferences, such as International Joint Conference on Artificial Intelligence (IJCAI) and Conference on Information and Knowledge Management (CIKM). 
	\end{IEEEbiography}
	
	\vspace{-1cm}
	\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{small_pics/saifu.jpg}}]{Sai-fu Fung}
		received the Ph.D. degree from the University of Warwick, Coventry, U.K. He is currently with the Department of Applied Social Sciences, City University of Hong Kong, Hong Kong. His current research interests include comparative methods and democratisation and politics
		of East and Southeast Asia.\end{IEEEbiography}
	
	\vspace{-1cm}
	\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{small_pics/guodong.png}}]
		{Guodong Long} was born in China. He received his Ph.D. degree in computer science from the University of Technology Sydney, Australia, in 2014.
		He is currently a Senior Lecturer and core member in the Centre for Artificial Intelligence (CAI), Faculty of Engineering and Information Technology, University of Technology Sydney, Australia. \par His research focuses on machine learning, data mining and cloud computing. 
	\end{IEEEbiography}
	
	
	\vspace{-1cm}
	\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{small_pics/jingjiang.png}}]
		{Jing Jiang}  is currently a Lecturer at the Centre for Artificial Intelligence, Faculty of Engineering and Information Technology at the University of Technology Sydney (UTS), Australia. She has a PhD degree in Information Technology. Her research interest lies in data mining and machine learning applications with the focuses on deep reinforcement learning and sequential decision-making.
	\end{IEEEbiography}
	
	\vspace{-1cm}
	\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{small_pics/chengqi.png}}]
		{Chengqi Zhang} received his Ph.D. degree from the University of Queensland, Brisbane, Australia, in 1991 and the D.Sc. degree from Deakin University, Geelong, Australia, in 2002.
		Since December 2001, he has been a Distinguished Professor of Information Technology with the University of Technology Sydney (UTS), Sydney, Australia, and he has been the Director of the UTS Priority Investment Research Centre for Quantum Computation and Intelligent Systems since April 2008. His research interests mainly focus on data mining and its applications. He is General Co-Chair of KDD 2015 in Sydney, the Local Arrangements Chair of IJCAI-2017 in Melbourne, a Fellow of the Australian Computer Society and a Senior Member of the IEEE. 
	\end{IEEEbiography}
